Black-Box Saliency Map Generation Using Bayesian Optimisation

Saliency maps are often used in computer vision to provide intuitive interpretations of what input regions a model has used to produce a specific prediction. A number of approaches to saliency map generation are available, but most require access to model parameters. This work proposes an approach for saliency map generation for black-box models, where no access to model parameters is available, using a Bayesian optimisation sampling method. The approach aims to find the global salient image region responsible for a particular (black-box) model's prediction. This is achieved by a sampling-based approach to model perturbations that seeks to localise salient regions of an image to the black-box model. Results show that the proposed approach to saliency map generation outperforms grid-based perturbation approaches, and performs similarly to gradient-based approaches which require access to model parameters.

==> glossary.tex <==
\renewcommand{\glossarypreamble}{This appendix provide a list of acronyms used in this study.}

% \cleardoublepage
% \ifpdf
% \phantomsection
% \fi

%\chapter{Acronyms}
\label{app:acronyms}

\newacronym{ml}{ML}{machine learning}
\newacronym{dl}{DL}{Deep learning}
\newacronym{ai}{AI}{artificial intelligence}
\newacronym{cnn}{CNN}{convolutional neural network}
\newacronym{nn}{NN}{neural network}
\newacronym{relu}{ReLU}{rectified linear unit}
\newacronym{fc}{FC}{fully-connected}
\newacronym{knn}{k-NN}{k-nearest neighbours}
\newacronym{svm}{SVM}{support vector machine}
\newacronym{hog}{HoG}{histograms of oriented gradients}
\newacronym{sift}{SIFT}{scale invariant feature transform}
\newacronym{csir}{CSIR}{Council for Scientific and Industrial Research}
\newacronym{mds}{MDS}{Modelling and Digital Science}
\newacronym{mias}{MIAS}{Mobile Intelligent Autonomous Systems}
\newacronym{sgd}{SGD}{stochastic gradient descent}
\newacronym{vgg}{VGG}{Visual Geometry Group}
\newacronym{eda}{EDA}{exploratory data analysis}
\newacronym{tsne}{t-SNE}{T-distributed stochastic neighbour embedding}
\newacronym{cam}{CAM}{class activation maps}
\newacronym{gp}{GP}{Gaussian process}
\newacronym{dli}{DLI}{Deep Learning Indaba}
\newacronym{wiml}{WiML}{Women in Machine Learning}
\newacronym{bai}{BAI}{Black in AI}
\newacronym{rl}{R0L}{reinforcement learning}
\newacronym{nlp}{NLP}{natural language processing}
\newacronym{pdf}{PDF}{probability density function}
\newacronym{ei}{EI}{expected improvement}
\newacronym{lcb}{LCB}{Lower Confidence Bound}
\newacronym{mse}{MSE}{mean squared error}
\newacronym{se}{SE}{squared exponential}
\newacronym{pi}{PI}{probability of improvement}
\newacronym{cpf}{CPF}{cumulative probability function}

%\printglossaries
